On the Masking-Friendly Designs for Post-Quantum Cryptography

Masking is a well-known and provably secure countermeasure against side-channel attacks. However, due to additional redundant computations, integrating masking schemes is expensive in terms of performance. The performance overhead of integrating masking countermeasures is heavily influenced by the design choices of a cryptographic algorithm and is often not considered during the design phase. In this work, we deliberate on the effect of design choices on integrating masking techniques into lattice-based cryptography. We select Scabbard, a suite of three lattice-based post-quantum key-encapsulation mechanisms (KEM), namely Florete, Espada, and Sable. We provide arbitrary-order masked implementations of all the constituent KEMs of the Scabbard suite by exploiting their specific design elements. We show that the masked implementations of Florete, Espada, and Sable outperform the masked implementations of Kyber in terms of speed for any order masking. Masked Florete exhibits a $73\%$, $71\%$, and $70\%$ performance improvement over masked Kyber corresponding to the first-, second-, and third-order. Similarly, Espada exhibits $56\%$, $59\%$, and $60\%$ and Sable exhibits $75\%$, $74\%$, and $73\%$ enhanced performance for first-, second-, and third-order masking compared to Kyber respectively. Our results show that the design decisions have a significant impact on the efficiency of integrating masking countermeasures into lattice-based cryptography.

==> note.tex <==
Jan-Pieter D'Anvers, Angshuman Karmakar Sujoy Sinha Roy, and Frederik Vercauteren. Saber: Module-LWR based key exchange, CPA-secure encryption and CCA-secure KEM. Africacrypt, 2018. (for Saber scheme)
Michiel Van Beirendonck, Jan-Pieter D'Anvers, Aangshuman Karmakar, Josep Balasch, and Ingrid Verbauwhede, "A Side-Channel Resistant Implementation of SABER," ACM Journal on Emerging Technologies in Computing Systems. (first order secure Saber)
Luk Bettale, Jean-Sébastien Coron, and Rina Zeitoun. Improved High-Order Conversion From Boolean to Arithmetic Masking. TCHES, 2018. (for B2A conversion)
Jean-Sébastien Coron, Johann Großschädl, and Praveen Kumar Vadnala. Secure Conversion between Boolean and Arithmetic Masking of Any Order. In CHES. Springer, 2014. (for A2B conversion)
Tobias Schneider, Clara Paglialonga, Tobias Oder, and Tim Güneysu. Efficiently Masking Binomial Sampling at Arbitrary Orders for Lattice-Based Crypto. Public Key Cryptography, 2019. (for CBD $\beta_μ$) 
Hannes Gross, David Schaffenrath, Stefan Mangard. Higher-Order Side-Channel Protected Implementations of KECCAK. DSD, 2017. (for G, XOF)
Joppe W. Bos, Marc Gourjon, Joost Renes, Tobias Schneider, and Christine van Vredendaal. Masking Kyber: First- and Higher-Order Implementations. IACR Cryptol. ePrint Arch., 2021. (for higher order comparison)

